Distributed Recursive Least-Squares: Stability and Performance Analysis

The recursive least-squares (RLS) algorithm has well-documented merits for reducing complexity and storage requirements, when it comes to online estimation of stationary signals as well as for tracking slowly-varying nonstationary processes. In this paper, a distributed recursive least-squares (D-RLS) algorithm is developed for cooperative estimation using ad hoc wireless sensor networks. Distributed iterations are obtained by minimizing a separable reformulation of the exponentially-weighted least-squares cost, using the alternating-minimization algorithm. Sensors carry out reduced-complexity tasks locally, and exchange messages with one-hop neighbors to consent on the network-wide estimates adaptively. A steady-state mean-square error (MSE) performance analysis of D-RLS is conducted, by studying a stochastically-driven `averaged' system that approximates the D-RLS dynamics asymptotically in time. For sensor observations that are linearly related to the time-invariant parameter vector sought, the simplifying independence setting assumptions facilitate deriving accurate closed-form expressions for the MSE steady-state values. The problems of mean- and MSE-sense stability of D-RLS are also investigated, and easily-checkable sufficient conditions are derived under which a steady-state is attained. Without resorting to diminishing step-sizes which compromise the tracking ability of D-RLS, stability ensures that per sensor estimates hover inside a ball of finite radius centered at the true parameter vector, with high-probability, even when inter-sensor communication links are noisy. Interestingly, computer simulations demonstrate that the theoretical findings are accurate also in the pragmatic settings whereby sensors acquire temporally-correlated data.

==> mydefs.tex <==
\usepackage{xspace,amsmath,epsfig,subfigure,theorem,times}
\input{mysymbol.sty}

\newtheorem{assumption}{\hspace{0pt}\bf AS\hspace{-0.15cm}}
\newtheorem{lemma}{\hspace{0pt}\bf Lemma}
\newtheorem{proposition}{\hspace{0pt}\bf Proposition}
\newtheorem{observation}{\hspace{0pt}\bf Observation}
\newtheorem{theorem}{\hspace{0pt}\bf Theorem}
\newtheorem{corollary}{\hspace{0pt}\bf Corollary}
\newtheorem{fact}{\hspace{0pt}\bf Fact}
\newtheorem{remark}{\hspace{0pt}\bf Remark}
\newtheorem{test}{\hspace{0pt}\it Test Case}
\newtheorem{definition}{\hspace{0pt}\bf Definition}

\def\proof  {\hspace{0pt}{\bf{Proof: }}}
\def\remark {\hspace{0pt}{\bf{Remark }}}

\def\brvh{\breve h}
\def \E   {{\rm E}}
\def \I   {{\bf 1}}
\def \db  { ~{\rm dB}}
\def \hq  { \hat{q} }
\def \hbq {\hat{{\bf q}}}
\def \htheta  { \hat{\theta} }
\def \hsigma  { \hat{\sigma} }
\def \btheta  { {\mbox{\boldmath $\theta$}} }
\def \bbtheta  { {\mbox{\boldmath $\theta$}} }
\def \bsigma  { {\mbox{\boldmath $\psi$}} }
\def \hbtheta { {\mbox{\boldmath $\hat{\theta}$}} }

\def \argumentone     {(\Delta_{1})}
\def \functionone     {\frac{q_1 \left(1-q_1\right) }{p_v^2\argumentone}}
\def \functiononeb    {\frac{q_1 \left(1-q_1\right) }{p_v^2\argumentone \Delta_{1}^2}}
\def \argumenttwo     {(\Delta_{2})}
\def \functiontwo     {\frac{q_2 \left(1-q_2\right) }{p_v^2\argumenttwo}}
\def \functiontwob    {\frac{q_2 \left(1-q_2\right) }{p_v^2\argumenttwo \Delta_{2}^2}}
\def \functiononetwo  {\frac {q_2 \left(1-q_1\right) }{p_v\argumentone p\argumenttwo}}
\def \functiononetwob {\frac {q_2 \left(1-q_1\right) }{p_v\argumentone p\argumenttwo \Delta_{1} \Delta_{2}} }
\def \deltak          {\frac{\tau_{k} - \theta}{\sigma}}
\def \argumentk      {(\Delta_k)}
\def \functionk      {\frac{q_k \left(1-q_k\right) }{p_v^2\argumentk}}

\def \error {e_a}
\def \Q     {F_v}
\def \bby   {{\mbox{\boldmath $\beta$}} }
\def \bbby  { \beta }
\def \calB  {{\cal B}}

